Cracking White-box DNN Watermarks via Invariant Neuron Transforms

Recently, how to protect the Intellectual Property (IP) of deep neural networks (DNN) becomes a major concern for the AI industry. To combat potential model piracy, recent works explore various watermarking strategies to embed secret identity messages into the prediction behaviors or the internals (e.g., weights and neuron activation) of the target model. Sacrificing less functionality and involving more knowledge about the target model, the latter branch of watermarking schemes (i.e., white-box model watermarking) is claimed to be accurate, credible and secure against most known watermark removal attacks, with emerging research efforts and applications in the industry. In this paper, we present the first effective removal attack which cracks almost all the existing white-box watermarking schemes with provably no performance overhead and no required prior knowledge. By analyzing these IP protection mechanisms at the granularity of neurons, we for the first time discover their common dependence on a set of fragile features of a local neuron group, all of which can be arbitrarily tampered by our proposed chain of invariant neuron transforms. On $9$ state-of-the-art white-box watermarking schemes and a broad set of industry-level DNN architectures, our attack for the first time reduces the embedded identity message in the protected models to be almost random. Meanwhile, unlike known removal attacks, our attack requires no prior knowledge on the training data distribution or the adopted watermark algorithms, and leaves model functionality intact.

==> tex/ack.tex <==
\section*{Acknowledgments}
We would like to thank the anonymous reviewers for their constructive comments and input to improve our paper. This work was supported in part by National Natural Science Foundation of China (61972099, U1836213,U1836210, U1736208), and Natural Science Foundation of Shanghai (19ZR1404800). Min Yang is a faculty of Shanghai Institute of Intelligent Electronics \& Systems, Shanghai Institute for Advanced Communication and Data Science, and Engineering Research Center of CyberSecurity Auditing and Monitoring, Ministry of Education, China. 


==> tex/orphanage.tex <==
%%% It contains sentences that I may use but currently not
scale weight of normalization layer and meanwhile adjusting the signs of related parameters in the preceding layer (e.g, a convolutional or linear layer). 


corroborate DeepSigns' effectiveness and applicability

utterly destroying 

copyright statement of the legitimate person or patty

real-valued vector or matrix

embeds the private passport during training and not distributes it to the end-users. 

Specifically, they first replace the BatchNorm in each \textit{ConvBlock} with group or instance normalization layer. And during the training epoch, 

the learning process aims to simultaneously achieve
two goals, of which the first is to minimize the original task
loss (e.g. classification accuracy discrepancy) when no passport
layers included (NW); and the second is to minimize the
combined loss function (Eq. 1) with passports regularization

Private passport is embedded but not distributed

Algorithm-wise, this multi-task learning is achieved by
alternating between the minimization of these two goals. The
successfully trained DNN model NWis then distributed to
end-users, who may perform network inference without the
need of passports. Note that this is possible since passport layers
are not included in the distributed networks. The ownership
verification will be carried out only upon requested by the law
enforcement, by adding the passport layers to the network in
question NW; sand detecting the embedded sign signatures
with unyielding the original network inference performances.
Compared with scheme V1, this scheme is easy to use for endusers
since no passport is needed and no extra computational
cost is incurred. In the meantime, this ownership verification
is robust to both removal attacks and ambiguity attacks. The
downside, however, is the requirement to access the DNN
weights and to append the passport layers for ownership
verification, i.e. the disadvantages of white-box protection mode
as discussed in [2]. Therefore, we propose to combine it with
trigger-set based verification that will be described next.




a threat where (former) staffs exposed/stole all the resources from the originator and it is a special case of ambiguity attacks

avoiding IP tracing





\if0
Even encrypted by homomorphic encryption or other secure multiparty computation techniques, the gradient of one user's data would unavoidably once be exposed to either other clients or the parameter server in plain texts, which leaves the attacker a novel attack window for user privacy disclosure. 

Several recent works also notice this vulnerable point of gradients in open-network distributed learning paradigms and provide various preliminary studies on the privacy of gradients, demonstrating to our community and the industry many alarming results. For example, 


which leaves a huge gap between our current knowledge of the privacy property of average gradient and its wide application in the real world.

the equivalence of the plausibility of a sus ccessful data reconstruction attack with the solvability of a large-scale sparse linear equation systems. 

It in practice usually brings much faster convergence of the learning process, less communication rounds in transmission, more efficient utilization of modern parallel computing devices \textit{et cetera.}  

 Our work for the first time shows these seeming coincidences indeed imply many fundamental aspects of gradient privacy.
 
 Compared with existing inference attacks, a successful data reconstruction attack is more threatening as it causes the full leakage of the client's private data whichever participates in the training process, and further facilitates the attacker to easily know either sensitive attributes or global properties of the victim's data.
 
 
 %% the optimal bound on single-sample reconstruction
  If somehow not, we show with the following corollary the reconstructed $X$ still lives in a very close neighborhood of the ground-truth input.

\begin{col}[Optimal Error Bound of Reconstruction]\label{col:optim_bound_single}
When the above uniqueness condition is not satisfied, the attacker can still reconstruct the label $Y$ exactly and recover $X$ within the following optimal error bound:
\begin{equation}
 \myworries{\text{(should be derived from the optimal error of LSE)}}
\end{equation}
\end{col}


Nevertheless, our attack algorithm, first prototyped on the FCN case and extended to the shallow and deep convolutional neural networks, is highly compatible with most types of the aforementioned ReLU networks.  

As an analogy, the activation pattern of Sample $\#2$ is $D_1=\text{diag}(0, 0, 1, 1), D_2=\text{diag}(0,1,0,1,1)$.

on cause existing attacks to show either unstable attack behaviors or unsatisfying attack effectiveness,


$$
\sum_{c=1}^{K}\overline{g}_c\frac{\partial{f_c}}{\partial{[W_H]_i}} \nonumber \\ 
= \sum_{c=1}^{K}\overline{g}_c\frac{\partial{[W_H]_c^{T}f_{H-1}}}{\partial{[W_H]_i}} = 
$$

, and when the following condition on the weight matrices is satisfied,
\begin{equation}
\myworries{\text{(something about the rank -- placeholder)}}
\end{equation}
the attacker can also precisely reconstruct the data X from its gradient with uniqueness.

In practice, we find the uniqueness condition is always satisfied for the learning model in different stages of the training phase, which in turn means the attacker can always prevail.

\myworries{In fact, we prove in Theorem B.1 that if the attacker cannot determine either of the two terms, it is computationally hard for the attacker to solve the gradient equation}. In other words,

On one hand, by combining the necessary and sufficient condition in Proposition \ref{prop:reconstruct_D} and Theorem B.1 on the hardness of solving the gradient equation without knowing neither the $\{\overline{g}_{c}^{m}\}_{m=1, c=1}^{M, K}$ nor the $\{D_i^{m}\}_{i=1, m=1}^{H, M}$, it is reasonable to utilize the condition on the existence of exclusively activated neurons to certificate the privacy of multi-sample gradient. More details on this aspect are provided in Section \ref{}.

On the other hand, if

%% to prove the hardness of data reconstruction when the plausibility condition is not satisfied

\subsubsection{Hardness of Multi-Sample Reconstruction}
\begin{theorem}
If the attacker cannot determine the activation patterns $(D_i^{m})_{i=1}^{H}$ for the $m$-th training sample $(X_m, Y_m)$, then the reconstruction error for the data input $X_m$ is larger than $\text{(some terms)}$
\end{theorem}
\begin{proof}
Under the above assumption, we show as follows, even if the ground-truth $\{(g_c^{m})_{c=1}^{K}\}_{m=1}^{M}$ and the activation patterns of other samples are fully known, the reconstruction error between the reconstructed input $X_m$ and the input $X_m^{*}$ is still large than a lower bound.

First, we formulate the gradient equation at the $i$-th layer, i.e.,
\begin{align}
\sum_{m=1}^{M}\sum_{c=1}^{K}\overline{g}_c^{m}(D_{i}^{m}W_{i-1}\hdots W_0X_m)([W_{H}]_c^{T}D_{H}^{m}\hdots{W_{i+1}D_{i+1}^{m}}) \nonumber \\ 
= M\overline{G}_i
\end{align}
into the form $AX = b$, where $A \in \mathbb{R}^{d_id_{i+1}\times{Md}}$, $b = M\overline{G}_i$, and $X^{T} = [X_1^{T}, \hdots, X_M^{T}]$.

As is known, for the equation $AX = b$ constructed from the ground-truth activation patterns, the ground-truth input $X^{*} = [X_1^{*}, \hdots, X_M^{*}]$ is the solution, which satisfies $AX^{*} = b$. Intuitively, we can consider the matrix $X$ is the operator that computes the summation of the gradients over all the training samples. Similarly, we denote the equation collected from an arbitrary activation pattern for the $m$-th sample as $A^{'}X = b$, with its solution as $X = [X_1^{*}, \hdots, X_m, \hdots, X_M^{*}]$. Therefore, we have
\begin{align}
\label{eq:norm_eq}
    \|(A - A^{'})X^{*}\|_2 = \|A^{'}X^{*} - A^{'}X\|_2 \nonumber\\ 
    \le \|A^{'}\|_2\|X^{*} - X\|_2 = \|A^{'}\|_2\|X_m^{*} - X_m\|_2
\end{align}
Hence, the reconstruction error is always larger than $\|(A - A^{'})X^{*}\|/\|A^{'}\|$ (for simplicity, we abbreviate $\|\cdot\|$ for the 2-norm $\|\cdot\|_2$). Next, to consider the worst-case reconstruction error, we would like to derive the maximum of $\|(A - A^{'})X^{*}\|/\|A^{'}\|$ when $X_m$'s unknown activation pattern changes over the feasible set described by Eq. \ref{eq:and_eq}. In other words, we want to lowerbound
\begin{equation}
    \max_{(D_i^{m})_{i=1}^{H}}\frac{\|(A - A^{'})X^{*}\|}{\|A^{'}\|}
\end{equation}
where $A^{'}$ depends on the activation pattern of $X_m$ and $\|A^{'}\| := \max_{\|x\| \le 1}\|A^{'}x\|$ is the operator norm induced from the 2-norm.

On the one hand, according to Theorem 3 and its extension in \cite{AllenZhu2019ACT}, we upperbound $\|A^{'}\|$ by
\begin{align}
    \|A^{'}\| := \max_{\|x\| = 1}\|A^{'}x\| \\
    \le \max_{\|x\| = 1}O(\sqrt{\frac{\sum_{c=1}^{K}\sum_{m=1}^{M}(g_c^{m})^{2}}{K}d_i{M}})
    \le O(M\sqrt{\frac{d_i}{K-1}})
\end{align}


On the other hand, we lowerbound the term $\max_{(D_i^{m})_{i=1}^{H}}\|(A - A^{'})X^{*}\|$ by 
\begin{align}
&\max_{(D_i^{m})_{i=1}^{H}}\|(A - A^{'})X^{*}\| \\ 
&=\max_{(D_i^{m})_{i=1}^{H}}\|(A_{:,md_0:(m+1)d_0} - A^{'}_{:,md_0:(m+1)d_0})X_m^{*}\| \nonumber \\
&\ge \|A_{:,md_0:(m+1)d_0}X_m^{*}\| \\ 
&= \|\frac{\partial{\ell(f(X_m^{*}), Y_m;W_i)}}{\partial{W_i}}\|
\end{align}
 where the ``greater than'' can be taken when the diagonal of the activation matrix at the $i$-th layer, i.e., $D_i^{m}$, used to derive $A^{'}$ is set as the difference between the union of the diagonal entries $\alpha_{i}^{m}$ of the boolean activation matrices of all the samples and that of the ground-truth activation matrix of $X_m$, i.e., $D_i^{m} = (\bigvee_{m=1}^{M}\alpha_{i}^{m}) - \alpha_i^{m}$.
 
Therefore, by replacing the bounds for each term above into 
Inequality \ref{eq:norm_eq} and combining the bound on each , we have the reconstruction error is always larger than the following lower bound in the worst case
\begin{equation}
    \|X^{*} - X\| \ge \frac{\sqrt{K-1}}{M\sqrt{d_i}}\|\frac{\partial{\ell(f(X_m^{*}), Y_m;W_i)}}{\partial{W_i}}\|
\end{equation}

show the exclusive activation condition in Proposition \ref{prop:reconstruct_g} is also a necessary condition for label reconstruction, or otherwise, any attacker who exploits the gradient equation for reconstruction is hard to prevail. Based on this result, we further have 


%% some useless statements
To recap, in Section \ref{sec:multisample_attack}, we have proved the condition that \textit{each data sample has at least two exclusively activated neurons in the last but one layer and at least one exclusively activated neuron at the other layers} is \textit{sufficient} for determining the activation pattern $\{D_i^{m}\}_{i=1}^{H}$ of each data sample $X_m$ with uniqueness. This is done by explicitly constructing the algorithm. 

\end{proof}


%% some technical results I don't want any more 



\noindent{$\bullet$ \textit{Proofs for  Corollary \ref{col:label_bottleneck}}}
\begin{proof}[For Proposition \ref{prop:reconstruct_g}]
In the main text, we have proved the sufficiency of at least one exclusively activated neuron at the last but one layer for determining $\{(g_c^{m})_{c=1}^{K}\}_{m=1}^{M}$. In this part, we turn to the necessity part. 

Assume $\{(g_c^{m})_{c=1}^{K}\}_{m=1}^{M}$ can be  uniquely determined when the $m$-th training sample $(X_m, Y_m)$ has no exclusively activated neuron at the $(H-1)$-th layer. First, we show that an attacker should still stick to the gradient equation of $W_H$ for determining, because, otherwise, if he/she introduces the gradient equations at other layers, there would be more new variables to solve than the number of equations added to the system. Hence, under the assumption above, we consider the analytic property of the gradient equation w.r.t. $W_H$ below. For each $c=1, \hdots, K$, $\sum_{m=1}^{M}\overline{g}_c^{m}f^{m}_{H-1} =  M[\overline{G}_H]_c$.

By multiplying both sides with $W_H$, we have 
\begin{equation}
    \sum_{m=1}^{K}\overline{g}_c^{m}f^{m}_{H} = MW_H[G_H]_c
\end{equation}
where, according to Eq. \ref{eq:softmax}, $f^{m}_H$ (abbrev. as $f^m$) satisfies: $p_c^{m} = \frac{\exp{f^{m}_c}}{\sum_{c=1}^{K}\exp{f_c^{m}}}$ and, according to Eq. \ref{eq:g_def}, $g_c^{m} = -1 + p_c^{m}$ if $c = Y_{m}$ else $g_c^{m} = p_c^{m}$. Therefore, the equation system above is only with the variables $\{(g_c^{m})_{c=1}^{K}\}_{m=1}^{M}$. However,      
\end{proof}



\noindent{$\bullet$ \textit{Proof Sketch for Proposition \ref{prop:reconstruct_D}}.}
In this part, we prove by contradiction this condition is also necessary for uniquely determining the activation patterns. Assume otherwise there exist a batch of training samples where the $m$-th sample $X_m$ has its activation pattern $(D_i^{m})_{i=1}^{H}$ that are not exclusively activated at the $i$-th layer (for a certain $i\in\{1, \hdots, H-1\}$) yet the activation patterns of each data sample in this batch are uniquely determined by the ground-truth gradient $(\overline{G}_i)_{i=0}^{H}$ (recall $\overline{G}_i$ denotes the gradient of the loss function w.r.t. the weight matrix $W_i$, which connects the $i$-th and the $(i+1)$-th layers). 

Denote the indices of the samples which activate the $j$-th neuron at the $i$-th layer as $\mathcal{I}(j)$. Following the above assumption, we have $|\mathcal{I}(j)| \ge 2$ for all the $j$-th neuron activated by $X_m$. Then, it is easy to ascertain that, for each $j$-th neuron, the cooridinatewise \textit{and} of the diagonal entries $\alpha_{i}^{m}$ of the boolean activation matrices of the samples indexed by $m \in \mathcal{I}(j)$ satisfy the following equation, $\bigvee_{m\in\mathcal{I}(j)}\alpha_{i}^{m} = \delta_{ij}$
where, similar to Criterion \ref{cri:determine_D_single}, the $d_{i+1}$-dim vector $\delta_{ij}$ tests whether the element in the $j$-th row of $G_{i}$ is non-vanishing or not. Formally, $(\delta_{ij})_k = 0$ if $(G_i)_{jk} = 0$, while otherwise $(\delta_{ij})_k = 1$. By collecting the equations as in Eq. \ref{eq:and_eq} for each $j$, we have an equation system on the activation matrices at the $i$-th layer, which however is ill-posed and has no unique solutions. Therefore, this gives a contradiction and we prove the necessity of the existence of at least one exclusively activated neuron for the first $H-1$ layers.


where $\text{cond}$ and $\sigma$ respectively denotes the conditional number and the smallest singular value of the linear operator $\nabla_{W_i}{\ell^{m}}$, the derivative operator of the $m$-th sample at the $i$-th layer, as defined in Eq. \ref{eq:grad_eq_fcn_single} (by replacing the activation patterns $D_0, \hdots, D_H$ with the reconstructed pattern of $X_m$)

%% the full table on the datasets
%% the table for listing the scenarios we consider in this paper
\begin{table}[ht]
  \begin{center}
    \caption{Datasets and model architectures in experiments.}
    \label{tab:scenarios}
    \scalebox{0.8}{
    \begin{tabular}{c|l|l|c|c}
    \toprule
       Domain & Dataset & Task & Input Size & Model \\
      \midrule
      \multirow{3}{*}{Benchmarks} & MNIST & \makecell{Hand-written Digits \\ (10-class, images)} & $(1,28,28)$ & FCN/LeNet\\ 
      & CIFAR-10 & \makecell{Objects \\ (10-class, images)} & $(3,32,32)$ & FCN/LeNet \\ 
      & ImageNet & \makecell{Objects \\ (1000-class, images)} & $(3,224,224)$ & Deep CNNs\\
      \midrule
    \multirow{2}{*}{Healthcare} & Texas-100 & \makecell{Clinical Procedure \\ (100-class, binary)} & $(600)$ & FCN \\ 
    & ISIC Skin Cancer & \makecell{Lesion Diagnosis \\ (9-class, images)} & $(3,224,224)$ & Deep CNNs\\
    \midrule
    \multirow{3}{*}{Misc.} & FaceScrub & \makecell{Face Recognition \\ (20-class, images)} & \makecell{$(3, 50, 50)$ \\ $(3, 224, 224)$} &  \makecell{LeNet \\ Deep CNNs} \\ 
    & Purchase-100 & \makecell{Shopping Profile \\ (100-class, binary)} & $(600)$ & FCN  \\
    & Location-100 & \makecell{Check-in Profile \\ (100-class, binary)} & $(446)$ &  FCN\\
    \bottomrule
    \end{tabular}}
  \end{center}
\end{table}


% Moreover, based on the analysis, we also point out the theoretical bottleneck and the plausibility condition of data reconstruction attacks, and design an efficient algorithm to alert potential data leakage from gradients produced by the client.   

 \textit{(b) From the defense viewpoint,} once the plausibility condition is broken, we prove theoretically the hardness of data reconstruction attacks from the multi-sample gradient and implement a practical alert algorithm which efficiently checks the validity of the plausibility condition. We hope this alert algorithm may serve as a useful indicator for measuring the risk of gradient leakage in open-network distributed learning paradigms and helping build the trust between entities in distributed learning systems. 
 
 
 %% alert on possible gradient leakage. i don't think it is necessary
 \noindent\textbf{Alert on Possible Gradient Leakage.} Based on our proposed sufficient condition on a successful data reconstruct attack in Proposition \ref{prop:reconstruct_D}, we devise an alert algorithm to check whether the produced gradient is vulnerable against potential reconstruction attacks. In detail, given a batch of training samples, the alert algorithm first forwards each single sample through the FCNN and records the activation states at each layer. Then, it computes the exclusively activated neurons w.r.t. each sample in a layerwise manner. Finally, the algorithm checks the validity of the sufficient condition according to the exclusively activated neurons.  In practice, the alert algorithm can be executed on the client side before the average gradient leaves the local device, which is expected to help the common users understand and recognize this new type of threats to their private data.
 
 , leaving several important empirical phenomenon remain uninterpreted. For example, they commonly observe the hardness of privacy attack always multiplies when (1) the number of samples to produce the average gradient (i.e., the batch size, increases) and (2) the size of the target model decreases, without, however, any further explanations on the causes behind. In fact, we find in these gaps actually hide several fundamental yet unknown aspects of what makes a successful data reconstruction attack, which may provide more insights on further mitigation studies. 
 
 The omitted proof for the necessity part of Proposition \ref{prop:reconstruct_D} can be found in Appendix \ref{sec:app:proof}.  
 
  For example, the famous \textit{back-propagation} algorithm \cite{Rumelhart1986LearningRB} is in essence specially designed for efficient calculations of the gradient for neural networks, while the widely-used optimizers like Adam \cite{Kingma2015AdamAM} and Adagrad \cite{Duchi2011AdaptiveSM}, encapsulated in various deep learning frameworks, can be roughly viewed as different approaches to better utilize the gradient in parameter updating for faster or stabler learning.  
  % \noindent\textbf{Real-World Threats on Gradient Privacy.}
%% to introduce the practical risk of gradient in a 
% In the past few years, due to privacy regulations on user data and the trend of distributed learning paradigms in open networks (e.g., Google's federated learning systems for keyboard prediction \cite{Konecn2016FederatedLS, Bonawitz2019TowardsFL}), the gradient, instead of the raw user data, is becoming the basic traffic in the communication channels of these systems, which may increase the risk of gradient being captured by man-in-the-middle. Even encrypted by homomorphic encryption or other secure multiparty computation techniques \cite{Bonawitz2019TowardsFL}, the gradient of one user's data would unavoidably once be exposed to either other clients or the parameter server in plain texts, which still leaves the potential attackers or honest-but-curious server a novel attack window for privacy disclosure.


From the practical aspect, most previous attacks are all based on solving the gradient equation above with optimization-based techniques, by minimizing, e.g., the L2 difference between the ground-truth gradient and the gradient computed from the variables. Formally, it corresponds to the following optimization problem

which, as observed by our experiments in Section \ref{sec:exp_result}, can be highly unstable and hard to converge in about half of the repetitive trials.

%% a discussion which may be redundant
 It is based on this equivalence that existing attacks develop a learning-based framework to approximate the solution to the gradient equation, which amazingly reached desirable reconstruction quality of about $8$ samples, despite the instability, from their average gradient. This phenomenon seems to state, the average gradient is not as safe as we expect, or, at least, it states an attacker could possibly separate out every single sample from this seemingly inseparable mixture. However, as the existing attacks are almost black-box, there is still very little known about how such an attack could be possible. 
 
 \footnote{The derivation is similar to the proof of Lemma 4.1 in \cite[Lemma 4.1]{Kawaguchi2016DeepLW}.} 
 
 
% we provide the first comprehensive theory-oriented privacy analysis of \textit{data reconstruction attacks}, a new yet threatening attack which exploits the gradient information and targets at reconstructing the whole training batch from the average gradient, on 

% Unlike preliminary studies which cover very limited scenarios in evaluation and adopt optimization-based approach, our study adopts a theory-oriented viewpoint to analyze various enablers underlying this attack, proposes a more effective attack algorithm, and provides extensive evaluations for different attacks on a wide range of application scenarios. 




%% this part I can briefly describe
%% which was once used to describe the reconstruction attacks on convolutional neural networks
\noindent$\bullet$ \textbf{Extension to Convolutional Neural Networks.} \label{sec:extension_conv}
Finally, we extend our proposed data reconstruction attack algorithm above to image classifiers with convolutional neural networks. It is worth to notice, most of the shallow and deep convolution neural network (CNN) for classification usually implement its last several layers as an FCN with ReLUs, which on one hand facilitates transfer learning, but also on the other hand eases data reconstruction attacks \footnote{Some architectures like ResNet would by default use only one linear layer as the classifier part instead of an FCN, while we find a theory-oriented reconstruction attack is still plausible. Details can be found in Appendix \ref{sec:approx}.}. We denote these CNN classsifiers explicitly as $f = h\circ{g}$, where $h$ is the feature extraction part which are mainly composed of convolutional and pooling operations, and $g$ is an FCN for classification. In detail, our attack pipeline on CNNs contains the following two stages,

\noindent{1)} At the first stage, we reconstruct the inputs to the fully connected component $g$. Based on our theory and algorithms on ReLU networks, it can be done with low reconstruction errors for both the single-sample and the multi-sample cases.

\noindent{2)} At the second stage, from the reconstructed last feature maps (i.e., the inputs to the FCN layer, denoted as $(F_m)_{m=1}^{M}$), we propose the following two different technical choices for reconstructing the training samples from the gradient.

$\bullet$ \textit{Deconvolution-Based Approach:} Following the inverse order of the feature extraction part $h$, we correspondingly build a deconvolutional neural network by using a transposed convolution operation \cite{Noh2015LearningDN}, which shares the same filters with the original convolution operation, to invert the output of the convolution, and using an upsampling operation to invert the output of the pooling operation. We can directly input the reconstructed feature map into the built deconvolution network to get the reconstructed training samples. With evaluations, we find this approach is especially effective and efficient for shallow CNNs like LeNet.  

$\bullet$ \textit{Hybrid Approach:} We propose to fuse the previous optimization-based approach with the recovered feature maps from our attack on the FCN part in the first stage, which corresponds to the following learning objective, $
\min_{X_i} D(\frac{1}{M}\sum_{i=1}^{M}\nabla_{W}\ell(f(X_i;W), \overline{Y}_i), \overline{G}) + \lambda\|h(x_m) - \overline{F}_m\|_1$, where the latter term aims at minimizing the L1 distance between the reconstructed input's feature map with the reconstructed ones, and the former term is to minimize the difference between the ground-truth gradient and the gradient computed from the variables. In practice, we implement the distance function $D$ as the cosine distance between the flattened gradient at each layer. It is worth to notice, different from existing learning-based methods, our hybrid approach also utilizes the reconstructed labels $\overline{Y}_i$ with our proposed attack on the FCN part, which makes our approach highly stable. Via extensive evaluations in Section \ref{sec:exp_result}, we empirically prove that our hybrid approach noticeably improves the attack effectiveness of previous optimization-based attacks on deep CNNs in the majority of test cases.     

% As a final remark, we provide supportive evidence in the evaluation part to validate that, \myworries{given a training batch, once the FCN part of a CNN does not satisfy the condition in Proposition \ref{prop:reconstruct_D}, existing learning-based attacks are neither able to reconstruct the training batch to a recognizable level.} In a future work, it would be a very meaningful direction to analytically establish the equivalence between the condition in Proposition \ref{prop:reconstruct_D} with the plausibility of data reconstruction attacks on convolutional neural network classifiers.

%% please I use this paragraph to simplify our study to omit the bias vector, which is unnecessary
In our analysis, we omit the bias terms in our analysis mainly for the simplification of notations. Without loss of generality, analytic results and attack algorithms in the remainder of this paper can be directly extended to ReLU networks with bias following the common practices in deep learning theory \cite{Goodfellow-et-al-2016}, i.e., by adding a constant neuron to each layer.  


%% the model architecture we once used 
\noindent\textbf{Shallow CNN.} For shallow CNNs, we choose the famous LeNet architecture \cite{LeCun1998GradientbasedLA}, which is commonly used on low-resolution images. A typical LeNet has its feature extraction module $g$ that consists of: one input layer, one convolutional layer (kernel size $6\times{6}$, $6$ output channels, $1$ stride), one max-pooling layer of size $2\times{2}$, one convolutional layer (kernel size $5\times{5}$, $16$ output channels, $1$ stride), one max-pooling layer of size $2\times{2}$, and has its classifier module $h$ as a $3$-layer FCN.  

\noindent\textbf{Deep CNNs.} Finally, to evaluate our methodology at a more practical level, we also provide extensive experiments on most popular deep CNNs of wide commercial usages, including ResNet-18 \cite{He2016DeepRL}, VGG-11 \cite{Simonyan2015VeryDC}, DenseNet-121 \cite{Huang2017DenselyCC}, AlexNet \cite{Krizhevsky2014OneWT}, ShuffleNet-v2-x0-5 \cite{Ma2018ShuffleNetVP}, Inception-V3 \cite{Szegedy2016RethinkingTI}, GoogLeNet \cite{Szegedy2015GoingDW}, MobileNet-V2 \cite{Sandler2018MobileNetV2IR}. For all these architectures except ResNet-18, we specify the classification module as a three-layer FCN which has a hidden layer of $4096$ neurons. We leave the classification module of ResNet-18 by default as a linear layer as in \cite{He2016DeepRL} for validating our alternative reconstruction algorithm in Appendix \ref{sec:approx}.


%% the discussion with a pigeonhole theorem on the bottleneck of label reconstruction 
In fact, as a corollary from Proposition \ref{prop:reconstruct_g}, according to the pigeonhole theorem, we have the following theoretical bottleneck  on the maximal number of reconstructable labels via our attack.

\begin{col}
\label{col:label_bottleneck}
Our data reconstruction attacks on an FCN with ReLU can recover for sure the labels of at most $d_{H}/2$ samples from the averaged gradient.
\end{col}
Although we still have not figured out whether this theoretical bottleneck on our algorithm is also applicable to any gradient-equation-based data reconstruction attacks, we do observe empirically in most cases our novel attack is the strongest in label reconstruction among existing attacks. Moreover, the proved bottleneck of our attack is already large. For example, for a typical FCN model on MNIST classification in Tensorflow's official tutorial, $d_H$ is $128$, which means our attack in the worst case can reconstruct the labels of $64$ samples for sure from their average gradient, while, as far as we know, existing attacks only has theoretical guarantees on reconstructing the label of one single sample for sure \cite{Zhao2020iDLGID}.


%% the visualization result for the multi-sample case on the skin cancer dataset 
\begin{figure}
\begin{center}
\includegraphics[width=0.5\textwidth]{img/isic_skin.png}
\caption{Reconstruction results of a batch of skin cancer imaging (of size $8$) from its gradient of a $(3072-500-9)$ FCN on ISIC skin cancer dataset, with the PSNR metric reported below each best-matching sample pair.}
\label{fig:fcn_mult_demo}
\end{center}
\end{figure}

%% discussion on the hardness of data reconstruction attacks
% At first glance, we may notice, to separate out the gradient of each single sample from their average is almost as ill-posed as recovering each summand from their summation \cite{Werschulz1987WhatIT}. Hence, is it neither possible for an attacker to reconstruct multiple samples from the average gradient? 

% Surprisingly, such an attack is proved to be practically possible.

%% discussion about the ablation study
Besides, we also provide rich ablation studies to demonstrate how the key factors of the deep learning system inherently influence the system's vulnerability against data reconstruction attacks, to serve as a complement to our analytical results

%% discussion of the limitation of existing attacks on the dataset choice 
 Meanwhile, their attacks are only conducted on a limited number of standard benchmark datasets from the machine learning community, which is insufficient for evaluating whether the threats from data reconstruction attack do ubiquitously exist for different scenarios. 
 
 
 
 %% First, we characterize the condition of uniqueness of reconstruction with the following theorem.
%% the theorem on unique reconstruction, which I think is not very useful right now
\begin{theorem}[Plausibility of Multi-Sample Attack]
\label{thm:unique_mult}
Under the conditions of Propositions \ref{prop:reconstruct_g} \& \ref{prop:reconstruct_D}, given a mini-batch of unknown samples $\{(X_i,Y_i)\}_{i=1}^{M}$, with the data $X_i$ from the problem space $\mathcal{X}$, when the attacker captures the ground-truth average gradients from an arbitrary ReLU network $f(X) = W_HD_{H}W_{H-1}...W_1D_1W_0X$ for $K$-class classification, with a cross-entropy loss, if the following structural condition is satisfied,
\begin{equation}\label{eq:equation_number}
K\text{tr}(D_H(X))+\sum_{i=0}^{H-1}\beta(\overline{G}_i) \ge M\dim{\mathcal{X}}
\end{equation}
then the attacker can always precisely reconstruct each data sample $X_i$, $Y_i$ from its gradient with uniqueness w.r.t. permutation of the sample index. Here, $\beta(\overline{G}_i) := \text{tr}(D_i(X))\text{tr}(D_{i+1}(X))$, which counts the number of non-zero coordinates in the captured gradient at the $i$-th layer. 
\end{theorem}


%% Statistics of Exclusivity Conditions in my previous version
In fact, we also do statistics on the proportion of training batches which satisfy the exclusive activation condition in three typical scenarios, i.e., FCN, LeNet and VGGNet with the last-but-one fully-connected layer of dimension $512$. The results are shown in Fig. \ref{fig:exclu_stat}, along $10$ training epochs. 
\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.5\textwidth]{img/exclu_stat.png}
\caption{Proportions of mini-batches satisfying the exclusive activation condition in CIFAR-10 over $10$ epochs of training.}
\label{fig:exclu_stat}
\end{center}
\end{figure}
As we can see, when the batch size is smaller than a certain threshold (about $8-10$ in these cases), the exclusive activation condition is satisfied in over $50\%$ of the batches. Strikingly, for LeNet, the threshold on the batch size doubles to $16$ and almost $80\%$ of the batches satisfy the exclusive activation condition when the batch size is smaller. Meanwhile, the proportion of risky batches even increases when the learning process goes on. These above phenomenons alarm the privacy risks of label leakage when the training batch behind the gradient is potentially separable at the granularity of the exclusively activated neurons.  It may be inspiring for future researches to consider to check the number of exclusively activated neurons in a batch for alerting the potential label leakage.  

\subsubsection{Impact of Training Phase}\label{sec:training} In the third part, we study how the attack effectiveness changes along the learning process. We train each model for $10$ epochs and conduct data reconstruction attacks on $10$ randomly sampled training batches at the beginning of each epoch. All the models converge after $10$ training epochs. The upper part of Fig. \ref{fig:training} presents the box-plot of the attack effectiveness in terms of PSNR between every single sample and its best-matching reconstruction. As we can see, with the learning progressing, the median values of the PSNRs show a trend of decline. According to Theorem \ref{thm:unique_mult}, behind the decline is the decreasing number of non-vanishing scalar gradients and the resulting underdetermined gradient equation. To validate this point, we collect and plot the non-sparsity of gradients (i.e., the ratio of gradient coordinates larger than $10^{-7}$). As is shown in the lower part of Fig. \ref{fig:training}, on all three scenarios, the change of the reconstruction quality roughly conforms to that of the gradient sparsity. From this experiment, an attacker seems to gain more advantages if he/she chooses the attack timing as the initial stage of the learning process, while system builders may adopt a stricter privacy mechanism on the gradient at the beginning of the learning process and gradually relax the protection mechanism later on for better efficiency and utility on the primary learning task.
\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.5\textwidth]{img/training.png}
\caption{Effectiveness of data reconstruction attacks and the non-sparsity of captured gradients in $10$ training epochs.}
\label{fig:training}
\end{center}
\end{figure}


%% Time complexity is not needed in this version
\section{Comparison of Time Complexity}\label{sec:app:time}
For our attack, we report the average time of accomplishing the attack once. For the optimization-based baselines, we report the average time cost until the loss function of each attack becomes stable within a $10^{-5}$ variance, which is the same termination condition for experiments on the attack effectiveness. Table \ref{tab:time_cost} below lists the average time costs over $10$ repetitive tests when the batch size is $8$, within the same environment described in the next section. As we can see, the time complexity of our attack is at a similar level as previous attacks and can be slightly more efficient for FCNs and shallow CNNs.    

\input{tex/time_cost_table.tex}


%% a prelude used to introduce the time complexity result 
Besides, we also provide a tentative comparison of the time cost for different attack approaches in Appendix \ref{sec:app:time}.


%% discussion on the coverage of our study
\noindent\textbf{On the Coverage of Our Study.} In this study, we slightly narrow down our focus to the family of neural networks with ReLUs. In fact, due to the observation that conventional activation functions such as \textit{sigmoid} or \textit{tanh} may cause the gradient explosion in deep neural networks \cite{Goodfellow-et-al-2016}, ReLU immediately becomes one of the commonest choices in many commercial architectures because its numeric stability even in very deep architectures. Moreover, extensive experiments on many popular neural network architectures and various application domains could to some extension justify the generality of our study. Although we admit our coverage may leave few well-known architectures in natural language processing (NLP) like Long-Short-Term-Memory (LSTM) out of our coverage, Melis et al. however recently point out that data reconstruction attack in NLP is indeed a much simpler case \cite{Melis2019ExploitingUF}: the attacker can immediately check the non-vanishing vectors in the gradient of the embedding table, a common architecture in most NLP models which caches an embedding vector for each word in the vocabulary, to determine the words present in the training batch. However, whether it is possible and how to recover the exact word order in each single sentence still remains an open problem to solve. It may be an interesting future direction to extend our analysis and attack algorithm to this scenario and other more.      

%% The necessity part, which I think is incorrect currently 
\noindent{$\bullet$ \textit{Proof Sketch for the Necessity Part of Proposition \ref{prop:reconstruct_D}}.}
In this part, we prove by contradiction this condition is also necessary for uniquely determining the activation patterns. Assume otherwise there exist a batch of training samples where the $m$-th sample $X_m$ has its activation pattern $(D_i^{m})_{i=1}^{H}$ that are not exclusively activated at the $i$-th layer (for a certain $i\in\{1, \hdots, H-1\}$) yet the activation patterns of each data sample in this batch are uniquely determined by the ground-truth gradient $(\overline{G}_i)_{i=0}^{H}$ (recall $\overline{G}_i$ denotes the gradient of the loss function w.r.t. the weight matrix $W_i$, which connects the $i$-th and the $(i+1)$-th layers). 

Denote the indices of the samples which activate the $j$-th neuron at the $i$-th layer as $\mathcal{I}(j)$. Following the above assumption, we have $|\mathcal{I}(j)| \ge 2$ for all the $j$-th neuron activated by $X_m$. Then, it is easy to ascertain that, for each $j$-th neuron, the cooridinatewise \textit{or} of the diagonal entries $\alpha_{i}^{m}$ of the boolean activation matrices of the samples indexed by $m \in \mathcal{I}(j)$ satisfy the following equation, 
\begin{equation}\label{eq:and_eq}
\bigvee_{m\in\mathcal{I}(j)}\alpha_{i}^{m} = \delta_{ij}
\end{equation}
where, similar to Criterion \ref{cri:determine_D_single}, the $d_{i+1}$-dim vector $\delta_{ij}$ tests whether the element in the $j$-th row of $G_{i}$ is non-vanishing or not. Formally, $(\delta_{ij})_k = 0$ if $(G_i)_{jk} = 0$, while otherwise $(\delta_{ij})_k = 1$. By collecting the equations as in Eq. \ref{eq:and_eq} for each $j$, we have an equation system on the activation matrices at the $i$-th layer, which however is ill-posed and has many different solutions (mainly because the \textit{or} operation is commutable). Therefore, this gives a contradiction and we prove the necessity of the existence of at least one exclusively activated neuron for the first $H-1$ layers.



\noindent{$\bullet$ \textit{Proof Sketch for Theorem \ref{thm:unique_mult}}.}
The proof idea is similar to Theorem \ref{thm:unique_single}. To ensure the uniqueness of solution to the gradient equation, we need the number of scalar equations no smaller than the number of unknown variables to solve. The former one is the total number of non-vanishing coordinates in the gradients of each layer, which, using the notion of activation matrices, is $K\text{tr}(D_H)+\sum_{i=0}^{H-1}\text{tr}(D_i(X))\text{tr}(D_{i+1}(X))$, while the number of variables is $M\dim{\mathcal{X}}$ for a batch of $M$ samples.

\begin{rmk}[PSNR and Recognizability]
For better intuitions about the numeric results, based on our and previous experimental observations \cite{Geiping2020InvertingG}, when the PSNR metric is over $6$, the reconstructed image is largely correct in color distributions and has a certain level of recognizable details. Meanwhile, a higher PSNR usually means more recognizable details. When PSNR is over $20$ per sample, the reconstruction results are highly recognizable for human observers. When PSNR is over $100$ or even $\infty$, the reconstruction is considered to be exact (e.g., Fig. \ref{fig:fcn_single_demo}).
\end{rmk}











\begin{figure*}
\begin{center}
\includegraphics[width=1.0\textwidth]{img/depth_width_suite.png}
\caption{The change of reconstruction accuracy when the width of the last ReLU layer varies (\textbf{Top}) and when the number of layers varies (\textbf{Bottom}).}
\label{fig:layer_width}
\end{center}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% THE PART ON THE SCALE OF EQUATION SYSTEMS 


\noindent{$\bullet$ \textbf{Scale of Leaked Gradient Information.}} In this part, we vary the proportion of the ground-truth gradients accessed by the adversary to analyze how the level of gradient information leakage impacts the reconstruction results. We set the target model as a $3$-layer FCNN ($d_0$-$512$-$K$). Specifically, we randomly choose $\beta$ proportion of weight parameters. After the loss vectors and the activation patterns are determined, we only allow the attack algorithm to use this part of gradients to form the linear gradient equation system. Fig. \ref{fig:scale} plots the changes of PSNR and MSE of our proposed attack algorithm when $\beta$ increases. 


\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.45\textwidth]{img/scale.png}
\caption{Impact of proportion of gradients accessed by the adversary on the reconstruction accuracy.}
\label{fig:scale}
\end{center}
\vspace{-0.2in}
\end{figure}

\noindent\textbf{Results \& Analysis.} As we can see from Fig. \ref{fig:scale}, with an increased proportion of gradient information accessed by the adversary, the performance of data reconstruction attacks is strengthened correspondingly. For example, when $\beta$ increases from $0.5\%$ to $6\%$, the PSNR on CIFAR-10 increases from $7.04$ (noisy) to over $20$ (highly recognizable). Fig. \ref{fig:scale_demo} in Appendix \ref{sec:app:datasets} provides the visualization results. This conforms to our statement in Theorem \ref{col:optim_bound_mult}: Once the sufficient exclusivity condition is satisfied, the MSE of data reconstruction attacks would decrease quadratically. 


Although our analytic results have unveiled the feasibility of data reconstruction from gradient under both lack and sufficiency of exclusivity, there is still a distance from the full picture on the mechanism and the limit of data reconstruction attacks on ReLU FCNNs, especially on the remaining cases when the neuron exclusivity state satisfies neither Condition I nor Condition II. Fig. \ref{fig:discussion}(a) \& (b) plot the ratio of mini-batches in CIFAR-10 which satisfies the sufficient exclusivity condition. With an increased batch size and a decreased layer width, the frequency of sufficient exclusivity decreases rapidly and the remaining exclusivity situations emerge. This result partially explains why existing attacks mainly report success for a mini-batch no larger than $8$ but overcome an unknown performance bottleneck when the batch size becomes larger and the network becomes shallower \cite{Zhu2019DeepLF, Geiping2020InvertingG, Zhao2020iDLGID}. In Fig. \ref{fig:discussion}(c), we further show the PSNR of Inverting on $1000$ random batches which do not satisfy Conditions I \& II. As we can see, although the PSNR is only slightly lower than that of Inverting on mini-batches of sufficient exclusivity (green dotted line). However, the best PSNR for the remaining cases is much lower than the PSNR our proposed attack algorithm attains for mini-batch of sufficient exclusivity. It remains unclear whether an effective data reconstruction attack can be constructed for the remaining cases as in Section \ref{sec:atk_case_a}, or whether the impossibility of unique reconstruction can be proved as in Section \ref{sec:def_case_b}, which is left as an open question for future research.



Based on Table \ref{tab:exp_full_table}, we suppose the adversary leverages the best baseline attack \textit{Inverting}, on the four scenarios where Inverting reconstructs meaningful results to some degree, namely, CIFAR-10, OrganMNIST, DermaMNIST and FaceScrub. According to the exclusivity reduction strategy in Corollary \ref{col:exclusivity_reduction}, we modify the original FCN architecture ($d$-$512$-$K$) to be ($d$-7-$512$-$K$), where the first hidden layer of width $7$ has no ReLU activation. Fig. \ref{fig:defense} plots the box-plot of the per-sample MSE and PSNR of Inverting on the target FCN with or without exclusivity reduction on four scenarios. 


\noindent\textbf{Results \& Analysis.} As we can see from Fig. \ref{fig:defense}, when we apply the exclusivity reduction strategy by inserting a linear layer into the original FCN, the PSNR on four datasets decreases by $25.7\%$ and the MSE increases by $49.4\%$ on average. To inspect the effectiveness of this strategy in a more intuitive way, we plot the reconstruction results of Inverting on the FCN with exclusivity reduction in Fig. \ref{fig:demo_defense}. Compared with the previous results in Fig. \ref{fig:demo}, the reconstructed images in Fig. \ref{fig:demo_defense} are more mixed with other samples in the same batch. For example, on FaceScrub each reconstructed face is observed to be much closer to the average of this batch of inputs than to their ground-truth counterpart. Combined with our observation in Section \ref{sec:evaluation} that a larger target FCN and more accessible gradient information tend to 
be more vulnerable against data reconstruction attack, the deterioration of reconstruction attacks on the slightly larger FCN (i.e.,  ($d$-7-$512$-$K$) vs. ($d$-$512$-$K$)) should be reasonably attributed to the reduced exclusivity. Although existing works have also considered general privacy protection mechanisms against data reconstruction attacks (e.g., differential privacy, gradient compression and sparsification \cite{Zhu2019DeepLF, Geiping2020InvertingG}), our preliminary study on controlling neuron exclusivity state aims at modifying the base mechanism of deep learning for better privacy, which we hope may provide novel insights on the privacy protection of gradients by design.  
%%%%%%%%%% BEGIN OF WIDTH_DEPTH CURVE
\begin{figure}
\begin{center}
\includegraphics[width=0.45\textwidth]{img/width_depth_suite_excerpt.pdf}
\caption{The PSNR curve of reconstruction attacks on DermaMNIST \textbf{Left:} when the width of the last ReLU layer and \textbf{Right:} when the number of layers varies.}
\label{fig:layer_width}
\end{center}
\end{figure}
%%%%%%%%%% BEGIN OF WIDTH_DEPTH CURVE


%%%%%%%%%%%%%%%%%% BEGIN OF FIG AC1 SIZE-ASR 
\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.45\textwidth]{img/ac1_size_asr_paper.pdf}
\caption{Impact of the batch size on the performance of our proposed attack on Facescrub.}
\label{fig:ac1_size_asr}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%% END OF FIG AC1 SIZE-ASR


%%%%%%%%%%%%%%%%%% BEGIN OF FIG AC3 EPOCH-ASR 
\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.45\textwidth]{img/ac3_iter_asr_paper.pdf}
\caption{Impact of the number of training epochs on the performance of our proposed attack on CIFAR-10.}
\label{fig:ac3_iter_asr}
\end{center}
\end{figure}
%%%%%%%%%%%%%%%%%% END OF FIG AC3 EPOCH-ASR
As an analogy to the single-sample case, to determine the $\{\overline{g}_c(X_m, Y_m)\}_{m=1, c = 1}^{M, K}$ and $\{D_i(X_m)\}_{m=1, i=1}^{M, H}$ in prior will reduce the gradient equation above to a system of linear scalar equations, which enables a successful data reconstruction attack by equation solving. 


the gradient comes onto the stage, which calculates as 
In other words, the gradient on the training sample is exactly the partial derivative of the loss function w.r.t. the model parameters. In many



a common choice for a wide range of $K$-class classification tasks with input features in vector forms. An input feature  typically comes from the dataset itself (e.g., a shopping record can be represented as a binary feature vector where each element denotes whether the corresponding item has been bought or not) or from the feature extraction part of most deep CNNs as in transfer learning \cite{Ji2018ModelReuseAO}. Also, 


Besides, ReLU is From FCNs to deep convolutional neural networks (CNN) like GoogLeNet \cite{Szegedy2015GoingDW} and ResNet \cite{He2016DeepRL}, a very broad class of popular neural network architectures are now implemented with the ReLU activation function (simply, ReLU). Concretely, a ReLU $\sigma(\cdot)$ can viewed as a gate structure which allows non-negative values to pass through without any change and meanwhile blocks negative values by outputting $0$ instead. Such a behavior is formally written as $
\sigma(x) = x$ if $x\ge{0}$; $\sigma(x)=0$ if $x<{0}$.



In this work, we mainly focus our analytical results on a fully-connected neural network (FCN) with rectified linear units (ReLU). It is a common choice for a wide range of $K$-class classification tasks with feature vectors in e.g., $\mathbb{R}^{d_0}$, which may come from the dataset itself (e.g., a shopping record can be represented as a binary feature vector where each element denotes whether the corresponding item has been bought or not) or from the feature extraction part of most deep CNNs as in transfer learning \cite{Ji2018ModelReuseAO}. 





By supposing the ground-truth gradient is calculated on an unknown mini-batch $\{(X_1, Y_1),\hdots, (X_M, Y_M)\}$, the gradient equation w.r.t. the parameter $W_i$ can be written as $\overline{G}_i = \frac{1}{M}\sum_{m=1}^{M}\sum_{c=1}^{K}\overline{g}_c(X_m, Y_m)\frac{\partial{f_c(X_m)}}{\partial{W_i}}$. 

For simplicity, we abbreviate $\overline{g}_c(X_m, Y_m), f_{H-1}(X_m)$ as and $f^{m}$. To recap, $f^{m} = D_H(X_m)W_{H-1}...D_1(X_m)W_0X_m \in \mathbb{R}^{d_{H-1}}$. Therefore, i

In general, if we form the ratio equations as in the single-sample case, the terms $f^{m}$ can not be canceled out, which makes it seemingly impossible to determine the ratios $\overline{g}_{c}^{m}$. However, 




%%%%%%%%%%%%%%%%%%% PREVIOUS DISCUSSIONS
 
\noindent\textbf{On the Threat Model.}
In general, our threat model assumes the attacker knows the gradient, the parameters and the architecture of the victim's FCNN. 

\noindent{$\bullet$ \textit{On the Parameters and the Architecture}}: It is a common situation in most distributed learning systems, where the clients and the parameter server share the same model architecture, and the server synchronizes with the client the global model parameter in a periodic manner. In this protocol, either a malicious client or a honest-but-curious parameter server can be the potential attacker in the threat model. Furthermore, the rationale of the assumption on random initialization is: Intuitively, if a model has been trained for epochs, the parameters itself would contain a certain level of knowledge about the training data, which allows an attacker to leverage other techniques, e.g., generative models \cite{Hitaj2017DeepMU, Salem2019MLLeaksMA}, to exploit the knowledge in the parameters to improve the reconstruction. Yet, mainstream implementations of data reconstruction attacks still use the gradients as the only information source \cite{Zhu2019DeepLF, Zhao2020iDLGID, Geiping2020InvertingG}.
As a result, to explain and understand data reconstruction attacks, we suppose the victim neural network is untrained and has random weights. We use the default random initialization scheme as in popular deep learning libraries (e.g., \cite{NEURIPS2019_9015}). 

\noindent{$\bullet$ \textit{On the Accessibility of the Gradients}}:  In existing distributed learning systems, secure multiparty computation is still an optional security strategy. As a result, when there is no protection over the gradient, even a man-in-the-middle attack in the open network may capture the gradient submitted by the victim who is participating in a distributed learning process. As the shape of the gradient itself encodes the structural information about the corresponding FCNN architecture, the man-in-the-middle would be able to infer the architecture accurately. Meanwhile, an honest-but-curious server may also play the adversary role in our threat model if the distributed learning protocol applies no secure aggregation algorithm  \cite{Bonawitz2019TowardsFL}. However, there do exist other distributed learning algorithms (e.g., FedAvg \cite{Konecn2016FederatedLS}) where, instead of the average gradient, the client submits its current parameters, after being locally updated for several times, to the server. Such a protocol is out of the coverage of our current analytic study. As a future work, it is meaningful to explore and evaluate the privacy risks of gradients or, in general, of visible intermediate model updates in more distributed learning paradigms. 



\noindent\textbf{Limitations and Future Directions.}
Despite the novel insights and results we present, we admit there still remain some unclear points towards the full picture of the privacy properties of gradients and its intrinsic relation with the deep learning practice.



%%%%%% EVALUATION DETAILS 
For single-sample cases, we simply apply the above two metrics on the reconstructed data input and the ground-truth. For multi-sample cases, as the attacker aims at reconstructing the orderless batch of data samples, we first leverage the Hungarian algorithm \cite{Kuhn1955TheHM} to find the best-matching pairs of reconstructed and ground-truth data inputs according to the pairwise MSE. Then we compute the average performance metrics over the best-matching pairs. 

For example, the reported MSE of our attack algorithm is smaller than $10^{-10}$ for the $M=1$ cases, which provides strong empirical evidences for Theorem \ref{thm:unique_single}. Meanwhile, for the $M = 8$ cases, our attack algorithm consistently outperforms all the baselines in both metrics by a large margin.


% In summary, under the condition of sufficient exclusivity, our constructed data reconstruction attack algorithm outperforms previous attacks and shows near-optimal reconstruction performance on most of the test cases, which empirically supports our analytical results in Section \ref{sec:atk_case_a}. Combining with the visualization results in Fig. \ref{fig:ac2_vgg_demo}, we conclude that our proposed hybrid attack does pose a more realistic threat to unprotected gradient information from a more wide range of neural network models. 

 \nonumber 
\\ \to W_H\sigma(W_{H-1}\hdots(W_1(W_0X+b_0)+b_1)\hdots+b_{H-1}) + b_H,

% \noindent{$\bullet$ \textit{On the Coverage of the Study:}} As is widely recognized \cite{Goodfellow-et-al-2016}, the ReLU FCNN architecture is a common choice for a diverse set of multi-classification tasks, which can take either original features from data or deep features from pretrained models (e.g., GoogLeNet or BERT \cite{Devlin2019BERTPO}) as inputs. As conventional activation functions including \textit{sigmoid} and \textit{tanh} would cause gradient explosion in deep neural networks \cite{Goodfellow-et-al-2016}, the past decade witnesses ReLU becoming one of the most popular activation functions due to its numeric stability. As a result, considering both its wide application and its mathematical conciseness, we choose this model family as the main focus of this study. It would be meaningful to explore the direction of extending our analysis and the attack algorithm to more complicated architectures including convolutional and recurrent neural networks. 


\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.4\textwidth]{img/facescrub.png}
\caption{Reconstruction results of a celebrity face from its gradient of a ($30000$-$500$-$20$) FCNN (from the FaceScrub dataset), with the reported PSNR. Compared with the experimental results of three existing attacks, our novel attack algorithm yields an almost near-optimal reconstruction quality.}
\label{fig:fcn_single_demo}
\end{center}
\end{figure}


\begin{figure*}
\begin{center}
\includegraphics[width=1.0\textwidth]{img/demo_defense.png}
\caption{Reconstruction results of the Inverting attack on the gradient of a random batch of $8$ samples from an FCNN with the first ReLU layer replaced as a linear layer, corresponding to the same settings of Fig. \ref{fig:defense}.}
\label{fig:demo_defense}
\end{center}
\end{figure*}




\noindent{$\bullet$ \textit{Proof for Theorem \ref{thm:unique_single}.}} The correctness of the label reconstruction in the single-sample case is obvious from Remark \ref{remark:label_reconstr} in our main text. To prove the exactness of reconstructing the data input, we consider the gradient equation w.r.t. $W_0$, which provides the attacker $\text{tr}(D_0)\dim{\mathcal{X}}$ linear scalar equations. These equations form an overdetermined linear equation system to solve for the unknown data input which contains only $\dim\mathcal{X}$ variables ($\le \text{tr}(D_0)\dim{\mathcal{X}}$). Moreover, 1) this linear equation system has the ground-truth data input in its solution set, which is also the least-square-error solution. 2) Under random initialization of the weights, the derivative operator is full-rank almost surely \cite{AllenZhu2019ACT}. Hence, by solving the system with least square error solver, the attacker will always find the ground-truth data input as the solution.   


When $D_1^m \equiv {D_1}$ for each $m$ (i.e., the lack of exclusivity), $A$ is always of full row rank almost surely if the weight is randomly initialized \cite{AllenZhu2019ACT}, which we formally state in our context as follows. 
\begin{lma}
If $W_0, \hdots, W_H$ are randomly initialized, i.e., each $W_i$ has i.i.d. entries respecting a Gaussian distribution $\mathcal{N}(0, \sigma_i^2)$, then the derivative operator $A$ is always of full row rank almost surely,
i.e., $\text{Pr}(\text{rank}(A) = M) = 1$.
\end{lma}
\begin{proof}
To prove, we consider the event $\text{Pr}(\text{rank}(A) < M)$ happens if and only if $A^{T}A$ is a singular matrix, which is equivalent to $\text{det}(A^{T}A) = 0$. Then, if we view the entries in $W_0, \hdots, W_H$ as variables, then $\text{det}(A^{T}A)$ reduces to a polynomial $p(W_0,\dots, W_H)$. Therefore, we have $\text{Pr}(\text{rank}(A) < M) = \int_{\{p(W_0,\dots, W_H)=0\}}p_0(W_0)\hdots{p_H(W_H)}dW_0\hdots{dW_H}$, where $p_i$ denotes the Gaussian probability density function of $W_i$. As the algebraic set $\{p(W_0,\dots, W_H)=0\}$ specified the polynomial equation has a Lebesgue measure zero, we prove $\text{Pr}(\text{rank}(A) < M) = 0$, which in other words implies $\text{Pr}(\text{rank}(A) = M) = 1$.
\end{proof}

As $A$ is of full row rank, $A^{\dagger}$ exists in the closed form $A^{T}(A^{T}A)^{-1}$.

After $\overline{g}_c^{m}$ is determined, the attacker can further determine the labels of the samples in the batch by checking the sign of the recovered $\{\overline{g}_c(X_m, Y_m)\}_{m=1, c = 1}^{M, K}$. 
\fi

In the past decades, deep learning begins to play a vital role in building modern intelligent systems on a wide variety of applications in the real world, such as autonomous driving[], finance[], healthcare[], and many more.

  

 In consideration of the growing training cost of large-scale high-performance deep neural networks (DNNs) models[] these years, the extensive computational resources, massive amounts of well-annotated training data, and the knowledge of deep learning experts become competitive leverage of the IT corporations. However, the malicious adversaries in real-world are more likely prone to illegally copy, redistribute or abuse the target model without authorization at a pretty lower cost, rather than training from scratch or purchasing from the legitimate model owners, which 
 
 Inspired by the digital watermarking schemes in Digital Rights Management[], a common approach to prevent copyright infringement of model IP is DNN watermarking. In a general model watermarking process, a secret identification information is first embedded into the model during the training stage, without noticeably impacting the performance of original models. Later, the ownership is verified by the detection of the same or similar watermarks extracted from the suspect model. 
 
 According to whether the full access to the suspect model (e.g. weights and activations of the hidden neurons) is required for model watermark recovery or not, DNN watermarking methods can be broadly categorized into two groups: black-box[] and white-box techniques.
As only the final output of the model is available during black-box watermarking verification, the secret information is embedded in the patterns of input-output pairs, which can be e-xtracted later from the remote intelligent systems by querying the model through the prediction API [] with a set of well-chosen inputs (i.e. trigger set). 
In the white-box setting, model watermark is embedded in the position-specific parameters or the inner activation maps, which consequently need the full access to the suspect model to determine the model ownership. 

% ################## overview ##################
% black-box decrease the acc while white-box increase the acc; complement for each other
Recent researches have indicated that black-box DNN watermarking techniques always inevitably decrease the model's performance slightly by changing the distribution of training dataset, while white-box watermarks can even increase the accuracy of original task by introducing some special regularizers in the training process. Moreover, these two groups of techniques can be regarded as a complement for each other[gan-wm]. 
For example, in the extreme situation when only a final model prediction is accessible from the suspicious online intelligent systems, the owner can first collect sufficient evidence by black-box watermarks verification, and then he can further claim the ownership of suspect model by white-box watermarking detection with law enforcement.

% ################## overview ##################
% removal attack: fine-tuning or input transformation
% ambiguity attack: cast doubt
% For example, several attacks attempt to remove the inside watermark of the model by carefully adjusting the model parameters (e.g. advanced fine-tuning methods[refit], or knowledge distillation []), while [parallel] transforming inference samples to invalidate the effects of watermark perturbations and patterns. Another line of works unveil the existence of ambiguity attacks by manufacturing counterfeit watermark to throw doubt on the ownership verification[].

% ################## overview ##################
% exist attacks to challenge the robustness of wm
% the limitation of previous attacks
% acc drop & prior knowledge (e.g. training data or wm algorithms) <- additional computing power?
% focus on black-box; white-box survive by strong correlation to significant parameters
% trend: whitr-box wm bring high credibility; robust whit-box are recently proposed
Nevertheless, growing security concerns about the robustness of these model IP protection techniques have raised. Some recent works explore attack strategies on confusing the model ownership verification process. Carefully performing the model post-processing techniques (e.g. fine-tuning or pruning[]), the secret information encoded in the watermarked model can be removed by disturbing the watermark-related parameters or the output of trigger set.
However, previous published works to invalidate the watermarking mechanisms suffer from some inherent restrictions. On the one hand, these attack methods are carried out with the sacrifice of model utility and certain prior knowledge to ensure the expected modification of the target model, e.g. the distribution of the whole or part of original training data[] or the details of specific model watermark's embedding algorithm[]. On the other hand, the majority of current attacks focus on black-box DNN watermarking verification and limited early white-box methods, as state-of-the-art white-box watermarking techniques have survived by virtue of the strong correlation to the significant parameters[] or stable selected activation maps[]. As a result, full access to the suspect model to acquire the inner weight matrices or hidden activation maps during ownership identification appears to bring higher credibility, as recently proposed white-box watermark methods have claimed the strong robustness against various attacks[].
% along with the unavoidable drop in adversarial utility and additional computing power which causing an unacceptable trade-off that violates the primary attack object.


(2) black-box is usually an alternative when sometimes the suspect model cannot be accessed as the ); (3) black-box can be removal by backdoor detection, while existing attempts on white-box won't work. 



In fact, existing attack attempts on white-box model watermarking works at a rather superficial level via popular model post-processing techniques (e.g., finetuning or pruning). By virtue of the strong correlation to the significant parameters[] or stable selected activation maps[], these attacks usually sacrifice too much on model utility until fully removing the embedded watermark from the model. 

to than black-box watermarking. On one hand, white-box verification by design involves much more knowledge about the suspect model, which ought to provide more accurate verification. For example, \cite{} suggests the owner first collect sufficient evidence by black-box watermarks verification, and then verify the ownership by white-box watermarking via law enforcement. On the other hand, by virtue of the strong correlation to the significant parameters[] and stable selected activation maps[], existing attacks via popular model post-processing techniques (e.g., ) usually sacrifice too much on model utility until fully removing the embedded watermark from the model. 

, illegally copying, redistributing and monetizing private DNN at a low attack budget. In face of model piracy, how to protect the intellectual property (IP) of DNN becomes an urgent open problem.
% from illegal duplication or reproduction. 


, and propose an effective removal attack which blindly cracks $8$ mainstream white-box watermarking scheme while leaving the model utility integral.   which leaves the original model functionality integral at almost no cost and is general to almost all the white-box watermarking algorithms. For the first time we empirically prove that \textit{all} the white-box watermarking algorithms rely heavily on the \textit{model intrinsic locality}, which is derived from position-specific parameters or the inner activation maps. By disturbing the model intrinsic locality of watermark-related model parameters, our attack based on model invariance invalid eight existing white-box watermarking techniques published at top-tier venues, indicating the enhancement to the connection between significant model parameters and watermark effectiveness gives the model owner a false sense of watermark security.


Specifically, the model with batch normalization layers is vulnerable to our attack (Section \ref{sec:dnn_invariance}).

% Zhang et al. \cite{zhang2020passportaware} propose another passport-aware normalization approach which is compatible with most known normalization layers. They mainly want to implement the passport-based watermark method without modifying the target network structure, which would otherwise incur notable performance drops. Specifically, they adopt a simple but effective strategy by training the passport-free and passport-aware branches in an alternating order and maintaining the statistic values independently for the passport-aware branch at the inference stage. Similar to DeepIPR, the authors design the learnable $\gamma, \beta$ to be relevant to the original model for stronger ownership claim. During the extraction of model watermarks, the transformation function $A$ first projects the $\gamma$ by an additional FCN model to an equal-length vector and then utilizes the signs of the vector to match the target signature.

==> tex/tables/intro_table_2.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t]
  \caption{Our attack strategy cracks $9$ mainstream white-box DNN watermarks \mytodo{(also compare with existing attacks. May use another table to compare the advantages of our attack.)}.}
    \centering
  \scalebox{0.8}{
    \begin{tabular}{ccccc}
    \toprule
    \multirow{2}[4]{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Equivalent Transformation}} & \multicolumn{1}{c}{\multirow{2}[4]{*}{\textbf{Our Unified Attack}}} \\
\cmidrule{2-4}          & \multicolumn{1}{c}{\textit{PathScale}} & \multicolumn{1}{c}{\textit{LayerShuffle}} & \multicolumn{1}{c}{\textit{SignFLip}} & \multicolumn{1}{c}{} \\
    \midrule
    Uchida's\cite{uchida2017embedding} & \ding{51}     & \ding{51}      & \ding{51}      & \ding{51}  \\
    \midrule
    RIGA\cite{wang2021riga}  & \ding{51}     & \ding{51}      & \ding{51}      & \ding{51}  \\
    \midrule
    Greedy Residuals\cite{liu2021greedyresiduals} & \ding{51}     & \ding{51}      & \ding{51}      & \ding{51}  \\
    \midrule
    IPR-GAN\cite{ong2021iprgan} & \ding{55}     & \ding{51}      & \ding{51}      & \ding{51}  \\
    \midrule
    Lottery Verification\cite{chen2021lottery} & \ding{55}     & \ding{51}      & \ding{55}      & \ding{51}  \\
    \midrule
    DeepSigns\cite{darvish2019deepsigns} & \ding{51}     & \ding{51}      & \ding{51}      & \ding{51}  \\
    \midrule
    IPR-IC\cite{lim2022ipcaption} & \ding{51}     & \ding{51}      & \ding{51}      & \ding{51}  \\
    \midrule
    DeepIPR\cite{fan2021deepip} & \ding{51}     & \ding{51}      & \ding{51}      & \ding{51}  \\
    \midrule
    Passport-aware\cite{zhang2020passportaware} & \ding{51}     & \ding{51}      & \ding{51}      & \ding{51}  \\
    \bottomrule
    \end{tabular}}%
  \label{tab:intro_table2}%
\end{table}%
